Scaling up Trustless DNN Inference with Zero-Knowledge Proofs

As ML models have increased in capabilities and accuracy, so has the complexity of their deployments. Increasingly, ML model consumers are turning to service providers to serve the ML models in the ML-as-a-service (MLaaS) paradigm. As MLaaS proliferates, a critical requirement emerges: how can model consumers verify that the correct predictions were served, in the face of malicious, lazy, or buggy service providers? In this work, we present the first practical ImageNet-scale method to verify ML model inference non-interactively, i.e., after the inference has been done. To do so, we leverage recent developments in ZK-SNARKs (zero-knowledge succinct non-interactive argument of knowledge), a form of zero-knowledge proofs. ZK-SNARKs allows us to verify ML model execution non-interactively and with only standard cryptographic hardness assumptions. In particular, we provide the first ZK-SNARK proof of valid inference for a full resolution ImageNet model, achieving 79\% top-5 accuracy. We further use these ZK-SNARKs to design protocols to verify ML model execution in a variety of scenarios, including for verifying MLaaS predictions, verifying MLaaS model accuracy, and using ML models for trustless retrieval. Together, our results show that ZK-SNARKs have the promise to make verified ML model inference practical.

==> tex/apx_protocols.tex <==
\section{Applications of Verified ML Model Inference}
\label{sec:apx-protocols}

In this section, we describe our protocols for verifying ML models for different
applications. We describe our security model and our protocols for verifying ML
model predictions for audits, verifying ML model accuracy, and verifying ML
model predictions for serving.


\subsection{Protocol Properties and Security Model}

\minihead{Protocol properties}
In this section, we describe and study the properties of protocols leveraging
verified ML inference. Each protocol has a different set of requirements, which
we denote $A$. The requirements $A$ may be probabilistic (e.g., the model has
accuracy 80\% with 95\% probability). We are interested in studying the
\emph{validity} of our protocols, which states that if the protocol completes,
$A$ holds.

For the accuracy verification and inference protocols, the parties can choose to
participate or not. As such, we are also interested in the \emph{rational
participation} of our protocols, which states that economically rational actors
will participate in our protocols.


\minihead{Security model}
In this work, we use the standard ZK-SNARK security model for the ZK-SNARKs
\cite{bunz2020transparent}. Informally, the standard security model states the
prover and verifier only interact via the ZK-SNARKs and that the adversary is
computationally bounded. This excludes the possibility of side channels. This is
in contrast to prior work in MPCs, which assume a semi-honest adversary (i.e.,
adversaries that honestly follow the protocol). Namely, adversaries may be
malicious in our security model.

We further assume the standard security model of public, permissionless,
Turing-complete smart contract execution engines (which are typically
blockchains) \cite{mohanta2018overview}. Informally, two parties can securely
send messages and execute smart contracts publicly. 


\minihead{Assumptions}
We require standard assumptions for ZK-SNARKs and smart contract execution
engines for our protocols to be secure.

For validity, we require that it is hard to compute the order of random group
elements \cite{bunz2020transparent}, which is implied by the RSA assumption
\cite{rivest1978method}. We further require the difficulty of finding hash
collisions, which is standard in cryptography \cite{rogaway2004cryptographic}.
Namely, for validity, we only assume standard cryptographic assumptions.

For rational participation, we assume that all parties are economically rational
and that there is an escrow service. We note that this excludes ``griefing''
attacks, where a malicious party purposefully loses money to hurt another party.
We defer the analysis of non-economically rational actors to future work. The
escrow service can be constructed programmatically, such as via smart contracts.
Importantly, the escrow service can also be run permissionlessly and trustlessly.




\subsection{Verifying ML model predictions for audits}
In this setting, a requester is interested in retrieving records that match the
output of an ML model from a responder. The responder is is typically the
subject of a legal subpoena. For example, the requester may be a journalist
requesting documents under the Freedom of Information Act or the plaintiff
requesting documents for legal discovery. For this setting, we assume that the
requester has a model that has been validated by some external party, e.g., a
judge. The responder must divulge documents or images that match the ML model's
prediction for the positive class but wishes to keep the remainder of the
documents private.

The protocol proceeds as follows:
\begin{enumerate}
  \item The responder commits to the dataset by producing hashes of the documents.
  \label{audit:hash}
  \item The requester sends the model to the responder.
  \item The responder produces ZK-SNARKs of the model on the documents, with the
  inputs hashed. The responder sends the requester the documents that match the
  positive class of the model.
\end{enumerate}

The audit protocol guarantees the following: the responder will return the
documents from Stage \ref{audit:hash} that match the model's positive class.
The validity follows from the difficulty of finding hash collisions and the
security of ZK-SNARKs.

The responder may hash invalid documents (e.g., random or unrelated images),
which the protocol makes no guarantees over. This can be mitigated in several
ways, depending on the scenario.

For documents from a trusted source, the hashes can be verified from a signature
from the trusted source. As an example, hashes for government-produced documents
(in the FOIA setting) may be produced at the time of document creation.

For documents from an untrusted source (e.g., the legal discovery setting), we
require a commitment for the entire corpus. Given the commitment, the judge can
allow the requester to randomly sample a small number ($N$) of the documents to
verify the hashes. In this case, the requester can verify that the responder
tampered with at most $p = \exp\left( \frac{1 - \delta}{N} \right)$ for some
confidence level $\delta$.



\subsection{Verifying ML model accuracy}
In this setting, a model consumer (MC) is interested in verifying a model
provider's (MP) model's accuracy, and MP desires to keep the weights hidden.
As an example use case, MC may be interested in verifying the model accuracy to
purchase the model or to use MP as an ML-as-a-service provider (i.e., to
purchase predictions in the future). Since the weights are proprietary, MP
desires to keep the weights hidden.

For this setting, we are interested in analyzing both the validity and rational
participation. As such, we analyze the pseudononymous marketplace setting, where
there are many potential MCs and MPs. We assume the existence of an escrow
service. This escrow service need only be able to follow programmatic rules and
as a result can be done trustlessly via smart contracts
\cite{kurtulmus2018trustless}. Other forms of escrow services are also viable.

Denote the cost of obtaining a test input and label to be $E$, the cost of
ZK-SNARKing a single input to be $Z$, and $P$ to be the cost of performing
inference on a single data point. We enforce that $E > Z > P$. Furthermore, let
$N = N_1 + N_2$ be the number of examples used in the verification protocol.
These parameters are marketplace-wide and are related to the security of the
protocol.

The marketplace requires MP to stake $1000 N_1 E$ per model to participate. The
stake is used to prevent Sybil attacks, in which a single party fakes the
identity of many MPs. Given the stake, the verification protocol is as follows
for some accuracy target $a$:
\begin{enumerate}
  \item MP commits to an architecture and set of weights (by providing the
  ZK-SNARK keys and weight hash respectively). MC commits to a test set $\{
  (x_1, y_1), ..., (x_N, y_N) \}$ by publishing the hash of the examples.

  \item MP and MC escrows $2 N E + \epsilon$, where $\epsilon$ goes to the
  escrow service.

  \item MP selects a random subset of size $N_1$ of the test set. If MC aborts
  at this point, MC loses the full amount in the escrow to MP. If MC continues,
  it sends the subset of examples to MP.

  \item MP chooses to proceed or abort. If MP aborts, MC loses $N_1 P$ of the
  escrow to MP and the remainder of the funds are returned to MC and MP.
  \label{verify:mp-fooled}

  \item MC sends the remainder of the $N_2$ examples to MP. If MP aborts from
  here on out, MP loses the full amount in the escrow ($2 N E$) to MC.

  \item MP sends SNARKs of the $N_2$ examples with outputs revealed. The weights
  and inputs are hashed.

  \item If accuracy target $a$ is met, MC pays $2 (N_1 P + N_2 Z)$. Otherwise,
  MP loses the full amount $2NE$ to MC.
\end{enumerate}

The verification protocol is valid because MP must produce the outputs of the ML
model as enforced by the ZK-SNARKs. MC can compute the accuracy given the
outputs. Thus, if the protocol completes, the accuracy target is met.

Rational participation further requires that the cost of the model or price of
post-verification purchased predictions is greater than $1000 N_1 E$. Rational
participation requires that honest MP/MC will participate and that dishonest
MP/MC will not participate.
% TODO
% Our analysis below assumes that MP and MC do not ``time out.'' We defer the
% full protocol, which includes a sub-protocol to mitigate one of the parties
% timing out, to the Appendix.

Consider the case of an honest MP. If MC is dishonest, it can economically gain
by having MP proceed beyond Stage \ref{verify:mp-fooled} and having MP fail the
accuracy target. Since MP chooses the subsets $N_1$ and $N_2$, they can be drawn
uniformly from the full test set. Thus, MP can choose to proceed only if $P(a
\textrm{ met} | N_1) > 1 - \alpha$ is such that expected value for MP is
positive, where $\alpha$ depends on the choice of $\epsilon$ (we provide
concrete instantiations for $\alpha$ and $\epsilon$ below). If MC is honest, MP
gains in expected value by completing the protocol, as its expected gain is
\[
  (1 - \alpha) (N_1 P + 2 N_2 Z - \epsilon) + \alpha N_1 P.
\]

Consider the case of an honest MC. Note that an economically rational MP is
incentivized to serve the model if it has a model of high quality. Thus, we
assume dishonest MPs do not have model that achieves the accuracy target. The
dishonest MP can economically gain by aborting at Stage \ref{verify:mp-fooled}
at least 1000 times (as $E > P$). MC can choose to participate with MP that only
has a failure rate of at most 1\%. In order to fool honest MCs, MP must collude
to verify invalid test sets, which costs $2 \epsilon$ per verification. MP must
have 99 fake verifications for one failed verification from an honest MC. Thus,
by setting $\epsilon = \frac{N_1 P}{99}$, dishonest MP will not participate. For
this choice of $\epsilon$, $\alpha > \frac{49 N_1 P}{49 N_1 P + 99 NE}$.

From our analysis, we see that honest MP and MC are incentivized to participate
and that dishonest MP and MC will not participate, showing rational
participation.


\input{tex/tables/eval-main}


\subsection{Verifying ML Model Predictions}

In this setting, we assume that MC has verified model accuracy and is interested
in purchasing predictions in the ML-as-a-service setting. We use the same
notation as above.

The serving verification procedure proceeds in rounds of size $K$ (i.e.,
prediction is served over $K$ inputs). MC is allow to contest at any point
during the round, but not after the round has concluded. Furthermore, let $K
\geq K_1 > 0$. The verification procedure is as follows:
\begin{enumerate}
  \item MC escrows $2KZ$ and MP escrows $\beta KZ$, where $\beta \geq 2$ is
  decided between MP and MC.

  \item MC provides the hashes for the $K$ inputs to the escrow and sends the
  inputs to MP ($x_i$). MP verifies the hashes.

  \item MP provides the predictions ($y_i$) to the inputs (without ZK-SNARKs) to
  MC. MC provides the hash of $\textrm{Concat}(x_i, y_i)$ to the escrow.

  \item If MC believes MP is dishonest, MC can contest on any subset $K_1$ of
  the predictions.

  \item When contested, MP will provide the ZK-SNARKs for the $K_1$ predictions.
  If MP fails to provide the ZK-SNARKs, then it loses the full $\beta ZP$.

  \item If the ZK-SNARKs match the hashes, then MC loses $2 K_1 Z$ from the
  escrow and the remainder of the funds are returned. Otherwise, MP loses the
  full $\beta ZP$ to MC.
\end{enumerate}

For validity, if MP is honest, MC cannot contest successfully and the input and
weight hashes are provided. Similarly, if MC is honest and contests an invalid
prediction, MP will be unable to produce the ZK-SNARK.

% TODO: timeouts
For rational participation, first consider an honest MP. The honest MP is
indifferent to the escrow as it receives the funds back at the end of the round.
Furthermore, all contests by MC will be unsuccessful and MP gains $K_1 Z$ per
unsuccessful contest.

For honest MC to participate, they must either have a method of detecting
invalid predictions with probability $p$ or they can randomly contest a $p$
fraction of the predictions. Note that for random contests, $p$ depends on the
negative utility of MC receiving an invalid prediction. As long as $\beta KZ$ is
large relative to $\frac{K Z}{p}$, then MC will participate.

